Faster Diffusion Sampling with Randomized Midpoints: Sequential and Parallel

Sampling algorithms play an important role in controlling the quality and runtime of diffusion model inference. In recent years, a number of works~\cite{chen2023sampling,chen2023ode,benton2023error,lee2022convergence} have proposed schemes for diffusion sampling with provable guarantees; these works show that for essentially any data distribution, one can approximately sample in polynomial time given a sufficiently accurate estimate of its score functions at different noise levels. In this work, we propose a new scheme inspired by Shen and Lee's randomized midpoint method for log-concave sampling~\cite{ShenL19}. We prove that this approach achieves the best known dimension dependence for sampling from arbitrary smooth distributions in total variation distance ($\widetilde O(d^{5/12})$ compared to $\widetilde O(\sqrt{d})$ from prior work). We also show that our algorithm can be parallelized to run in only $\widetilde O(\log^2 d)$ parallel rounds, constituting the first provable guarantees for parallel sampling with diffusion models. As a byproduct of our methods, for the well-studied problem of log-concave sampling in total variation distance, we give an algorithm and simple analysis achieving dimension dependence $\widetilde O(d^{5/12})$ compared to $\widetilde O(\sqrt{d})$ from prior work.

==> Sections-Main-Body/experiments.tex <==
%\section{Experiments}
%
%
%
%
%\begin{figure}[h!]
%    \centering
%    \begin{subfigure}[b]{0.02\textwidth}
%        \rotatebox{90}{\textbf{DDIM}}
%    \end{subfigure}%
%    \begin{subfigure}[b]{0.24\textwidth}
%        \includegraphics[width=\textwidth]{experiment_images/ddim_stable_diffusion/ddim_output_10_steps.png}
%    \end{subfigure}
%    \begin{subfigure}[b]{0.24\textwidth}
%        \includegraphics[width=\textwidth]{experiment_images/ddim_stable_diffusion/ddim_output_20_steps.png}
%    \end{subfigure}
%    \begin{subfigure}[b]{0.24\textwidth}
%        \includegraphics[width=\textwidth]{experiment_images/ddim_stable_diffusion/ddim_output_30_steps.png}
%    \end{subfigure}
%    \begin{subfigure}[b]{0.24\textwidth}
%        \includegraphics[width=\textwidth]{experiment_images/ddim_stable_diffusion/ddim_output_40_steps.png}
%    \end{subfigure}
%
%    \begin{subfigure}[b]{0.02\textwidth}
%        \rotatebox{90}{\textbf{Randomized Midpoint}}
%    \end{subfigure}%
%    \begin{subfigure}[b]{0.24\textwidth}
%        \includegraphics[width=\textwidth]{experiment_images/randomized_midpoint_stable/stable_diffusion_rnd_midpoint_10_steps.png}
%    \end{subfigure}
%    \begin{subfigure}[b]{0.24\textwidth}
%        \includegraphics[width=\textwidth]{experiment_images/randomized_midpoint_stable/stable_diffusion_rnd_midpoint_20_steps.png}
%    \end{subfigure}
%    \begin{subfigure}[b]{0.24\textwidth}
%        \includegraphics[width=\textwidth]{experiment_images/randomized_midpoint_stable/stable_diffusion_rnd_midpoint_30_steps.png}
%    \end{subfigure}
%    \begin{subfigure}[b]{0.24\textwidth}
%        \includegraphics[width=\textwidth]{experiment_images/randomized_midpoint_stable/stable_diffusion_rnd_midpoint_40_steps.png}
%    \end{subfigure}
%
%    \begin{subfigure}[b]{0.02\textwidth}
%        \hspace{0.02\textwidth} % Aligns NFEs text with the images
%    \end{subfigure}%
%    \begin{subfigure}[b]{0.24\textwidth}
%        \centering
%        \caption*{10 NFEs}
%    \end{subfigure}
%    \begin{subfigure}[b]{0.24\textwidth}
%        \centering
%        \caption*{20 NFEs}
%    \end{subfigure}
%    \begin{subfigure}[b]{0.24\textwidth}
%        \centering
%        \caption*{30 NFEs}
%    \end{subfigure}
%    \begin{subfigure}[b]{0.24\textwidth}
%        \centering
%        \caption*{40 NFEs}
%    \end{subfigure}
%\end{figure}



==> d_sublinear_scratch.tex <==
\section{No Lipschitzness}
Let's try to bound
\begin{align*}
    \E\|\grad \ln q_{t_0 - \alpha h}(x_{t_0 - \frac{1}{2}}) - \grad \ln q_{t_0 - \alpha h}(x_{t_0}^*(\alpha h))\|^2
\end{align*}
We have
\begin{align*}
    &\frac{d}{dt} \E\| \grad \ln q_{t_0 - t} (x_{t_0 - \frac{1}{2}}) - \grad \ln q_{t_0 - t}(x_{t_0}^*(t))\|^2\\
    &= \frac{d}{dt} \E \|\grad \ln q_{t_0 - t}(x_{t_0 - \frac{1}{2}})\|^2 - 2 \frac{d}{dt}\inner{\grad \ln q_{t_0 - t}(x_{t_0 - \frac{1}{2}}), \grad \ln q_{t_0 - t}(x_{t_0}^*(t))} + \frac{d}{dt} \E\|\grad \ln q_{t_0 - t}(x_{t_0}^*(t))\|^2\\
    &= 
\end{align*}

\begin{align*}
    &\frac{d}{dt} \E\|\grad \ln q_{t_0}(x_{t_0}) - \grad \ln q_{t}(x_t)\|^2\\
    &= \frac{d}{dt} 2 \inner{ \grad \ln q_{t_0} (x_{t_0}), \grad \ln q_{t}(x_t)} + \frac{d}{dt} \inner{\grad \ln q_t (x_t), \grad \ln q_t(x_t)}
\end{align*}
\begin{lemma}
    \begin{align*}
        \frac{d}{dt} \grad \ln q_{t_0 - t}(x_{t_0}^*(t)) = -\grad\left( \Delta \ln q_{t_0 - t}(x_{t_0 - t})\right) - \grad \ln q_{t_0 - t}(x_{t_0 - t}) - \grad^2 \ln q_{t_0 - t}(x_{t_0 - t}) \cdot \grad \ln q_{t_0 - t}(x_{t_0 - t})
    \end{align*}
\end{lemma}
\begin{proof}
    We know
    \begin{align*}
        \frac{d}{dt} x_{t_0 - t} = x_{t_0 - t} + \grad \ln q_{t_0 - t}(x_{t_0 - t})
    \end{align*}
    Thus,
    \begin{align*}
        \frac{d}{dt} \grad \ln q_{t_0 - t}(x_{t_0}^*(t)) = \frac{d}{ds} \grad \ln q_{t_0 - s}(x_{t_0}^*(t))]_{s = t} + \frac{d}{ds} \grad \ln q_{t_0 - t}(x_{t_0}^*(s))]_{s = t}
    \end{align*}
    Now,
    \begin{align*}
        \frac{d}{ds} \grad \ln q_{t_0 - t} (x_{t_0}^*(s)) = \grad^2 \ln q_{t_0 - t}(x_{t_0 - s}) \left( x_{t_0 - s} + \grad \ln q_{t_0 - s}(x_s)\right)
    \end{align*}
    For the first term, the Fokker-Planck equation gives us:
    \begin{align*}
        \frac{d}{dt} q_{t_0 - t}(x) = - \grad \cdot ((x + \grad \ln q_{t_0 - t}(x)) q_{t_0 - t}(x))
    \end{align*}
    So,
    \begin{align*}
        \frac{d}{dt} \log q_{t_0 - t}(x) = \frac{\frac{d}{dt} q_{t_0 - t}(x)}{q_{t_0 - t}(x)} = -d - \Delta \ln q_{t_0 - t}(x) - \inner{x + \grad \ln q_{t_0 - t}(x), \grad \ln q_{t_0 - t}(x)}
    \end{align*}

    So,
    \begin{align*}
        \frac{d}{dt} \grad \ln q_{t_0 - t}(x) = - \grad(\Delta \ln q_{t_0 - t}(x)) - \grad \ln q_{t_0 - t}(x) - \grad^2 \ln q_{t_0 - t} x - 2 \grad^2\ln q_{t_0 - t}(x) \grad \ln q_{t_0 - t}(x)
    \end{align*}
\end{proof}

\section{$d$-Sublinear bound -- Predictor Step}

\begin{lemma}
    \label{lem:f_t_time_derviative}
    Let $f_t = f * w_t$, for distribution $f$ over $\R^d$, where $w_t$ is the pdf of $\mathcal N(0, t \cdot I_d)$. Let $x = x_0 + z \sim f_t$ for $x_0 \sim f$ and $z \sim w_t$.
    We have that
    \begin{align*}
        \frac{d}{dt} \grad \ln f_t(x) = \E\left[ \frac{z}{t^2} | x\right] - \E\left[\frac{ z \cdot \|z\|^2}{2t^3} | x \right] + \E\left[\frac{\|z\|^2}{2t^2} | x \right]\E\left[\frac{ z}{t} | x\right]
    \end{align*}
\end{lemma}
\begin{proof}
    By Tweedie's formula,
    \begin{align*}
         \grad \ln f_t(x) = \E\left[\frac{- z}{t} | x \right] = \int \frac{- z}{t} \cdot \frac{f(x - z) w_t(z)}{f_t(x)} dz
    \end{align*}
    We have
\begin{align*}
    \frac{d}{d t} w_t(z) = w_t(z) \left(-\frac{d}{2t} + \frac{\|z\|^2}{2t^2} \right)
\end{align*}
So,
\begin{align*}
    \frac{d}{d t} f_t(x) = \int f(x - z) \frac{d}{d t} w_t(z) dz = - \frac{d \cdot f_t(x)}{2t} + f_t(x) \cdot \E\left[\frac{\|z\|^2}{2 t^2} | x \right]
\end{align*}
So,
\begin{align*}
    \frac{d}{d t} \frac{f(x - z) w_t(z)}{f_t(x)} = \frac{f(x-z) w_t(z) \cdot \left(\frac{z^2}{2 t^2} - \E\left[\frac{z^2}{2t^2} | x \right] \right)}{f_t(x)}
\end{align*}
So finally,
\begin{align*}
    \frac{d}{d t} \grad \ln f_t(x) = \E\left[\frac{z}{t^2} | x \right] - \E\left[\frac{z \cdot \|z\|^2}{2t^3} | x\right] + \E\left[\frac{\|z\|^2}{2t^2} | x \right]\E\left[\frac{ z}{t} | x \right]
\end{align*}
\end{proof}

\begin{lemma}[Reparameterization]
    For distribution $q_t$ such that $q_t(y) \propto f_{e^{2t}-1}(e^t y)$, we have
\end{lemma}
\begin{proof}
    \begin{align*}
        \frac{d}{dt} \grad \ln q_t(y_t) = e^t \grad \ln f_{e^{2t} - 1}(x_{e^{2t} - 1}) + e^t \frac{d}{ds} \grad \ln f_s(x_s)]_{s = e^{2t} - 1} \cdot 2 e^{2t}
    \end{align*}
    So by Lemma~\ref{lem:f_t_time_derviative}, we have
    \begin{align*}
        \frac{d}{dt} \grad \ln q_t(y_t) = e^t \grad \ln f_{e^{2t} - 1}(x_{e^{2t} - 1}) + 2e^{3t} \cdot \E\left[\frac{z}{(e^{2t} - 1)^2} \right] 
    \end{align*}
\end{proof}

\begin{lemma}
    Consider the reverse ODE
    \begin{align*}
        \dot x_{t_0 - t} = x_{t_0 - t} + \grad \ln q_{t_0 - t}(x_{t_0-t})
    \end{align*}
    We have that
    \begin{align*}
        \frac{d}{dt} \grad \ln q_{t_0 - t}(x_{t_0 - t}) = \frac{d}{ds} \grad \ln q_{t_0 - s}(x_{t_0 - t})]_{s = t} + \grad^2 \ln q_{t_0 - t} (x_{t_0 - t}) \left(x_{t_0 - t} + \grad \ln q_{t_0 - t}(x_{t_0 - t}) \right)
    \end{align*}
\end{lemma}
\begin{proof}
    We have that
    \begin{align*}
        \frac{d}{dt} \grad \ln q_{t_0 - t}(x_{t_0-t}) = \frac{d}{ds} \grad \ln q_{t_0 - s}(x_{t_0-t})]_{s = t} + \frac{d}{ds} \grad \ln q_{t_0 - t}(x_{t_0-s})]_{s = t}
    \end{align*}
    Now, by the definition of the ODE,
    \begin{align*}
        \frac{d}{ds} q_{t_0 - t}(x_{t_0 - s}) = \grad^2 \ln q_{t_0 - t}(x_{t_0 - s})\left(x_{t_0 - s} + \grad \ln q_{t_0 - s}(x_{t_0 - s}) \right)
    \end{align*}
    The claim follows.
\end{proof}

\section{Scratch}

\begin{align*}
    \|\grad^2 \ln q_{t}(x_t) \cdot \grad \ln q_t(x_t)\|^2 = \| \E_{Z | x}\left[Z Z^T \right] \cdot \E_{Z|x}\left[Z \right]\|^2 = \E_{Z|x}\left[ Z\right]^T \E_{Z|x}\left[ZZ^T \right]^2 \E_{Z | x}\left[Z \right]
\end{align*}

Want to bound
\begin{align*}
    \E\|\E[Z Z^T | x]^2\| \le \E[\Tr(\E[ZZ^T | x]^2)] \propto \E[\Tr(\E[ZZ^T|x])]
\end{align*}
\begin{lemma}
    \begin{align*}
        \frac{d}{dt} \grad \ln q_{t_0 -  t} (x_{t_0 - \frac{1}{2}}) = 
    \end{align*}
\end{lemma}
\begin{proof}
    We know
    \begin{align*}
        x_{t_0 - \frac{1}{2}} = e^{t} x_{t_0} + \int_{t_0 - t}^{t_0} e^{s - (t_0 - t)} \grad \ln q_{t_0} (x_{t_0}) ds
    \end{align*}
    So,
    \begin{align*}
        \frac{d}{dt} x_{t_0 - \frac{1}{2}} = x_{t_0} e^t  + 
    \end{align*}
\end{proof}
SCRATCH
\begin{align*}
    \frac{d}{dt} \int_0^t e^{-\gamma(t - s)}\grad f(x_s) dt &= \frac{1}{\eps}\left(\int_{0}^{t + \eps} e^{-\gamma(t+\eps - s)} \grad f(x_s) ds - \int_0^t e^{-\gamma(t - s)} \grad f(x_s) ds\right)\\
    &= \frac{1}{\eps} \left(\int_t^{t+\eps} e^{-\gamma(t + \eps - s)}\grad f(x_s) ds + \int_{0}^t -e^{-\gamma(t-s)}\gamma \eps \grad f(x_s) \right)\\
    &= \grad f(x_t) - \gamma \int_0^t e^{-\gamma (t-s)}\grad f(x_s) ds
\end{align*}

\begin{align*}
    \frac{d}{dt} \int_0^t e^{-\gamma(t - s)} dB_s = 1 - \gamma \int_0^t e^{-\gamma(t - s)} d B_s
\end{align*}

Thus, we have
\begin{align*}
    d v_t &= -\gamma v_0 e^{-\gamma t} - u\left(\grad f(x_t) - \gamma \int_0^t e^{-\gamma(t - s)} \grad f(x_s) ds \right) + \sqrt{2 \gamma u} \left(1 - \gamma \int_0^t e^{-\gamma (t - s)} d B_s \right)\\
    &= -\gamma v_t - u \grad f(x_t) + \sqrt{2 \gamma u} dB_t
\end{align*}
\begin{align*}
    e^{-\gamma(t + \eps - s)} - e^{-\gamma(t - s)} = e^{-\gamma(t - s)} (e^{-\gamma \eps} - 1) =
\end{align*}
